Sailing Through Point Clouds: Safe Navigation Using Point Cloud Based Control Barrier Functions

The capability to navigate safely in an unstructured environment is crucial when deploying robotic systems in real-world scenarios. Recently, control barrier function (CBF) based approaches have been highly effective in synthesizing safety-critical controllers. In this work, we propose a novel CBF-based local planner comprised of two components: Vessel and Mariner. The Vessel is a novel scaling factor based CBF formulation that synthesizes CBFs using only point cloud data. The Mariner is a CBF-based preview control framework that is used to mitigate getting stuck in spurious equilibria during navigation. To demonstrate the efficacy of our proposed approach, we first compare the proposed point cloud based CBF formulation with other point cloud based CBF formulations. Then, we demonstrate the performance of our proposed approach and its integration with global planners using experimental studies on the Unitree B1 and Unitree Go2 quadruped robots in various environments.

==> old_preview.tex <==
However, checking the collision between the many paths and the environment may still be computationally expensive. Therefore, we propose to only use one path whose heading is a parameter that can be chosen such that the path is collision-free. To find this collision-free configuration, we can treat the path as a virtual robotic manipulator and the heading is determined by its joint angles. Using this abstraction, we can treat the problem of planning a safe trajectory over a time horizon as a collision-free inverse kinematics problem which can be solved efficiently using a CBFQP-based approach. To find this collision-free configuration, we deploy an iterative approach. First, we start from a joint configuration $\theta$ and compute the position and orientation of each link of the virtual robotic manipulator using forward kinematics. Note that the resulting position and orientation of the links will be with respect to the body frame of the robot, which means they are in the same frame as the point cloud data. Then, we compute the CBFs $\bm{h}_i(\theta)$'s, their partial derivatives $\partial\bm{h}_i(\theta)/\partial\theta$s, and solve the following CBFQP
\begingroup
\allowdisplaybreaks
\begin{align}
\label{eq:cbfqp_preview}
    \min_{\dot\theta}\ &\ \|\bm{J}_{ee}(\theta)\dot{\theta} - \dot{\bm{p}}_{ee}^\star\|_2^2\\
    \text{subject to}\ &\ \frac{\partial\bm{h}_i(\theta)}{\partial\theta}\dot{\theta} \geq -\Gamma(\bm{h}_i(\theta))\nonumber
\end{align}
\endgroup
where $\bm{p}_{ee} \in \mathbb{R}^3$ represents the end-effector position of the virtual robotic manipulator, $\dot{\bm{p}}_{ee}^\star \in \mathbb{R}^3$ the desired end-effector velocity, $n_\theta\in\mathbb{N}$ the number of joints, and $\bm{J}_{ee} \in \mathbb{R}^{6\times n_\theta}$ the end-effector Jacobian. The value of $\dot{\bm{p}}_{ee}^\star$ is computed as
\begin{equation}
    \dot{\bm{p}}_{ee}^\star = \bm{K}_p(\bm{p}^\star - \bm{p}_{ee})
\end{equation}
with $\bm{K}_p\in\mathbb{R}^{3\times3}$ being a diagonal gain matrix and $\bm{p}^\star$ the target configuration. After solving the CBFQP in~\eqref{eq:cbfqp_preview}, we update the joint configuration using
\begin{equation}
    \theta \leftarrow \theta + \eta\dot{\theta}^\star
    \label{eq:theta_update}
\end{equation}
where $\eta\in\mathbb{R}_+$ is a predefined step size and $\dot{\theta}^\star \in \mathbb{R}^{n_\theta}$ is the solution to~\eqref{eq:cbfqp_preview}. The procedure described in~\eqref{eq:cbfqp_preview} and~\eqref{eq:theta_update} is performed iteratively until convergence or a predefined maximum number of iterations has been reached. This process is also described in Algorithm~\ref{alg:preview}. The local target is then computed as
\begin{equation}
\label{eq:B_x_target_star}
    {}^\mathcal{B}\bm{p}_\text{target}^\star = \begin{bmatrix}
        l\cos(\theta^\star) & l\sin(\theta^\star) & 0.0
    \end{bmatrix}^\top
\end{equation}
with $l\in\mathbb{R}_+$ represents the length of the preview arm, ${}^\mathcal{B}\bm{p}_\text{target}^\star\in\mathbb{R}^3$ represents the position of the local target when measured in the robot body frame, and $\theta^\star\in\mathbb{R}$ is the output of Algorithm~\ref{alg:preview}. The preview control method is illustrated in Fig.~\ref{fig:preview_concept_visualization}. Note that the preview controller can be run at a much lower frequency than the CBFQP controller which ensures the safety of the robot body.
\begin{rem}
    Since the virtual robotic manipulator has a similar function as the needle on a compass, in the remainder of this paper, we refer to this preview control method as \textit{\textbf{Compass}} and the virtual robotic manipulator as the \textit{\textbf{needle}}.
\end{rem}
\input{preview_alg}
\begin{rem}
    The joint angle of the needle itself might also get stuck in a local equilibrium. Inspired by~\cite{Starke20}, this can be resolved by sampling a set of initial joint angles and running Algorithm~\ref{alg:preview}. Then, we can pick the solution closest to the current needle joint angle to ensure motion consistency.
\end{rem}
